Memory-Efficient LLM Training with Online Subspace Descent

Recently, a wide range of memory-efficient LLM training algorithms have gained substantial popularity. These methods leverage the low-rank structure of gradients to project optimizer states into a subspace using projection matrix found by singular value decomposition (SVD). However, convergence of these algorithms is highly dependent on the update rules of their projection matrix. In this work, we provide the \emph{first} convergence guarantee for arbitrary update rules of projection matrix. This guarantee is generally applicable to optimizers that can be analyzed with Hamiltonian Descent, including most common ones, such as LION, Adam. Inspired by our theoretical understanding, we propose Online Subspace Descent, a new family of subspace descent optimizer without SVD. Instead of updating the projection matrix with eigenvectors, Online Subspace Descent updates the projection matrix with online PCA. Online Subspace Descent is flexible and introduces only minimum overhead to training. We show that for the task of pretraining LLaMA models ranging from 60M to 7B parameters on the C4 dataset, Online Subspace Descent achieves lower perplexity and better downstream tasks performance than state-of-the-art low-rank training methods across different settings and narrows the gap with full-rank baselines.

==> tex/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our theoretical and empirical results align with our main claims.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed the limitation and difficulty in analyzing the class of method theoretically.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are clearly stated in the body of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Hyperparameters choices are provided and later we will make code publicly available anonymously.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All dataset and codebase used in the experiments are opensourced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All hyperparameters, including learning rate, rank of projectors, sequence length are specified in each experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:\answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training LLM is expensive, we can afford running multiple runs on large models. However, previous empirical studies have shown that variation across seed is generally small in language model pretraining.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: GPU type used in experiment is specified.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We comply with the Code of Ethnics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper aims to promote deeper theoretical understanding of a class of method. The algorithm itself is not practical enough to produce powerful enough LLM that could potentially have any negative societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: same reasoning as above
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Everything is opensourced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new asset has been introduced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No human subject has been invovled.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not perform any studies involving human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> tex/method_old.tex <==
\section{Dynamic Subspace Descent}

\subsection{Static Subspace Descent}
Consider the optimization problem of 
$$
\min_{\x}  L(\x). 
$$
Assume that we solve the problem with certain optimizer 
\bb 
\w_{t+1} =  W_t + \epsilon \phi(S_t, \w_t), 
&& 
 S_{t+1} = S_t + \epsilon  \psi(S_t, \W_t, G_t). 
\ee 
The problem is that the optimizer state $S_t$ could be memory costly. 

We consider a reparameterization that restricts the optimization into an low dimensional dimension. Let $\W = U \hat W $, for which we have 
$$
\min_{\hat W} L(U \hat W). 
$$
Note that $\hat G = \dd_{\hat W} L(U \hat W) = U\tt \dd_{W} L(W) = U\tt G$. 
Applying the same optimizer on $\hat W$, yields 
\bb 
 W_{t+1} = W_t + \epsilon  U \phi(S_t, U^+ W_t), 
&& 
 S_{t+1} =  S_{t} + \epsilon \psi(S_t, U \tt G_t). 
\ee 
where $U^+$ is the pseudo inverse of $U$ with $U^+ U = I$, 
such that $\hat W = U^+ W$.

\begin{exa}
When the optimizer is the simple gradient descent, we have 
$W_{t+1} = W_t + \epsilon U U\tt G_t$. 
\end{exa}

\begin{exa}
When the optimizer is heavy ball method, we have 
\bb 
\hat G_t = U\tt \dd f(W_t), &&
\hat M_{t+1} = \beta_t \hat M_t +  (1-\beta_t) \hat G_t , && 
W_{t+1} = W_t + \epsilon_t U M_t . 
\ee 
\end{exa}

However, with a static $U$, the optimization is restricted to a lower dimensional space and hence does not solve the original optimization. 

It is hence desirable to vary $U$ across iterations, such that optimization can be conducted in different subspaces across different iterations. Let $U_t$ be the projection matrix at iteration $t$,  
\bb 
 W_{t+1} = W_t + \epsilon  U_t \phi(S_t), 
&& 
 S_{t+1} =  S_{t} + \epsilon \psi(S_t, U_t \tt G_t). 
\ee 
%We proposal 

\subssection{Lyapunov Anaysis}
Let us consider 
$$
\dot W_t  = U_t \phi(W_t), ~~~~ \dot S_t = \psi(S_t, U_t \tt \dd L(W_t))
$$
\bb 
\ddt H(W_t, S_t) =\dd_W H w
\ee

\bb 
\dot W_t =   U_t \tt  \dd_S H(w_t, m_t) - \phi_t(\dd_W H(w_t, m_t))  \\
\dot S_t = -   U_t \dd_W H(w_t, m_t) + \psi_t(\dd_S H(w_t, m_t)) 
\ee 

Implicit: 
\bb 
\dd_x H =  V_m - V_x  \\
\dd_m H =  +V_x - V_m
\ee 
Then, 
$$
\dot H 
= \dd_x H\tt V_x + \dd_m H \tt V_m  
= (V_m - V_x)\tt  V_x + (V_x - V_m) V_m 
= 0.
$$

\begin{exa}
Consider the momentum method: 
\bb 
\dot x_t = - m_t, && \dot m =a (\dd f(x_t) - m_t). 
\ee 
The projected version is 
\bb
\dot x_t = U_t m_t , && \hat g_t = U_t\tt  \dd f(x_t), && \dot m_t = a (\hat g_t - m_t). 
\ee 
It yields a Lyapunov function of form
$$
H(x, m) = a f(x) + \frac{1}{2}\norm{m}_2^2. 
$$
for which we have 
\bb 
\ddt H(x_t, m_t) 
& = - a \dd f(x_t) \tt U_t m_t + a m_t\tt (U_t \dd f(x_t) - m_t) \\
& = - a \norm{m_t}_2^2\leq0.
\ee 
\end{exa}

\begin{exa}
Consider Adam, we have 
\bb 
\dot x_t = \frac{m_t}{\sqrt{v_t}+e},   && 
\dot m_t = a(\dd f(x_t) - m_t), && \dot v_t = b(\dd f(x_t)^2 - v_t). 
\ee 
The projected version is 
\bb 
\dot x_t =  U_t \frac{m_t}{\sqrt{v_t}+e},   &&  \hat g_t =  U_t \tt \dd f(x_t), && 
\dot m_t = a(\hat g_t - m_t), && \dot v_t = b(\hat g_t^2 - v_t). 
\ee 
It yields a Lyapunov function 
$$
H(x, m, v) = a f(x) + \frac{1}{2}  \left(\frac{1}{\sqrt{v} +e}\right)\tt m^2. 
$$
for which $\ddt H(x_t, m_t, v_t) \leq 0$ when $a \geq \frac{b}{4}$: 
\bb 
\ddt H(x_t, m_t, v_t) 
& = a g_t \tt U_t \frac{m_t}{\sqrt{v_t}+e}
+ a \left(\frac{m}{\sqrt{v} + e}\right) \tt (U_t\tt  g_t - m)
-  \frac{b}{4} \left(\frac{m^2}{ \sqrt{v}(\sqrt{v} + e)^2} \right)\tt (\hat g_t^2 - v_t)  \\ 
& = 
- \left ( a - \frac{b}{4}\frac{\sqrt{v}}{\sqrt{v} + e}
\right )\tt \frac{m^2}{\sqrt{v }+ e}
-  \frac{b}{4} 1\tt \left(\frac{m^2 \hat g_t^2}{ \sqrt{v}(\sqrt{v} + e)^2} \right)   \\ 
& \leq \left(a - \frac{b}{4}\right) 1 \tt \frac{m^2}{\sqrt{v }+ e} - \frac{b}{4} 1\tt \left(\frac{m^2 \hat g_t^2}{ \sqrt{v}(\sqrt{v} + e)^2} \right) \leq 0, 
\ee 
where we assume $a \geq b/4$. 
\end{exa}

\section{$U_t$ Updates} 
We want to choose $U_t$ to conduct an online PCA. 

Derivation: We hope the reconstructed gradient $U_t U_t\tt g_t$ to be close to $g_t$ as much as possible. Hence, ideally, $u_t$ should minimizes the following objective function: 
\bb 
L_{g_t}(u) = \norm{u u \tt g_t - g_t}^2 + \gamma \norm{u \tt u - I}^2.  
\ee 
Remark: it is equivalent to replace $\norm{u\tt u - I}^2$ with $\norm{u \tt u - I}^2$, as they are equivalent upto a constant. 

We hence update $u_t$ by minimizing $L_t(u)$ in an online fashion. Hence, the simplest option is  $\dot u_t = - \dd L_t(u_t)$, but we can consider to use  any optimizer that receives the gradient $g^u_t = L_t(u_t)$ at  iteration $t$.

Properties of $L_g$: 
\begin{lem} 
Consider 
$$
L(u) = \frac{1}{2}\left(\norm{u u \tt g - g}^2 + \gamma \norm{u  u\tt - I}^2 \right).  
$$
Gradient:
\bb 
\dd L(u) 
= (u u \tt g - g) u g\tt 
+ g\tt  (u u \tt g - g) 
\ee 
$u$ is a set of orthogonal basis of the top $k$ eigenspace, 
iff it is global optimal solution, iff it is stable local optima. 
%Its global optimum solution
\end{lem}
\begin{proof}
It is known that $u$.  
\end{proof}


\begin{lem}
Let $u \in \RR^{k\times \ell}$,  then 
$$
\norm{u \tt u - I_\ell}^2 - \ell   = \norm{u u\tt - I_k}^2 - k. 
$$
The memory is 
\end{lem} 
\begin{proof}
\bb
\norm{u \tt u - I_\ell}^2  - \ell 
& = \trace(( u \tt u - I_\ell)\tt(u\tt u - I_\ell)) - \ell \\
& = \trace(u \tt u u \tt u - 2 u \tt u ). 
\ee 
%%
\bb 
\norm{u u \tt - I_k}^2  - k 
& = \trace(( u u \tt - I_k)\tt(u u\tt  - I_k)) - k \\
& = \trace(u u\tt  u u \tt  - 2 u u \tt ) \\ 
& = \trace(u\tt  u u \tt  u  - 2 u\tt u )\\
& = \norm{u \tt u - I_\ell}^2  - \ell. 
\ee 
\end{proof}

\subsection{Toy example}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/toy.png}
    \caption{Optimization trajectory of Rosenbrock function $f(x_1, x_2) = (1 - x_1)^2 +  10 \cdot (x_2 - x_1^2)^2$}, notice that Dynamic Subspace Descent provides a smoother optimization trajectory than Galore.
    \label{fig:toy}
\end{figure}

==> tex/method_v2.tex <==


\section{Dynamic Projected Descent}

\todo{outline here.}


\paragraph{Notation}
For matrices $\vv A, \vv B$, define 
$\llangle\vv A, \vv B\rrangle = \trace(\vv A\tt \vv B)$, 
and $\norm{A}^2 = \trace(\vv A \tt \vv A).$
We use $A\odot B$ to denote the elementwise product, 
and $A^{\odot2} = A\odot A $. 

%Consider the optimization problem of 
\subsection{Optimization Background}
The training of deep learning models reduces to an optimization problem 
$$
\min_{\vv\w}  L(\vv\w), 
$$
where $\vv \w$ the set of weight matrices of the model.  For simplicity, we assume $\vv \w \in \RR^{n\times m}$ is a single matrix of size $(n,m)$ without loss of generality. 
%%The optimization problem is solved with  optimizers such as stochastic gradient descent, momentum and Adam, 
\begin{exa}
Update rules of common optimizers: 
\begin{flalign*}
\text{Gradient Descent}:&~~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t \dd L(\vv W_t),&& &&&&&  \\ 
\text{Momentum}: & ~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t \vv M_t, &&
\vv M_{t} = (1-\beta) \dd L(\vv W_{t}) + \beta \vv M_{t-1}, &&&&&  \\
\text{Adam}:&~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t 
\frac{\vv M_t}{\sqrt{\vv V_t} + e}, &&
\vv M_{t} = (1-\beta_{1t}) \dd L(\vv W_{t}) + \beta_{1t} \vv M_{t-1}, &&&&&  \\
&&& 
\vv V_{t}= (1-\beta_{2t}) \dd L(\vv W_{t})^{\odot 2} + \beta_{2t}\vv V_{t-1},  &&&&& 
\end{flalign*}
where $\epsilon_t$ are step sizes, 
$A^{\odot 2} = A\odot A $ is the elementwise square, 
and $\vv M_t, \vv V_t$ are the first and second order momentum, 
and 
$\beta,\beta_{1t},\beta_{2t}$ are momentum coefficients in $(0,1)$, with $\beta_{it}=\frac{\beta_i - \beta_i^t}{1-\beta_{i}^t}$, $i=1,2$ for $\beta_1,\beta_2\in(0,1)$
in Adam.
%where $\eta_{it} = 1-\beta_{i}^t$ for Adam. 
\end{exa}
These optimizers can be unifiedly viewed as updating  $\vv W_t$ together with an  optimizer state $\vv S_t$: % across iteration $t$: 
%consisting of iterative update of form 
\bbb \label{equ:opt}
\vv w_{t+1} = \vv W_t +  \phi_t(\vv S_t), 
&& 
 \vv S_{t} =  \psi_t(\vv S_{t-1},  \dd L(\vv W_{t})), 
%\vv w_{t+1} = \vv W_t +  \phi_t(\vv S_t, \vv w_t), 
% \vv S_{t+1} =\vv S_t +   \psi_t(\vv S_t, \vv W_t, \dd L(\vv W_t)). 
\eee  
with some mapping $\phi_t, \psi_t$. 
We have $\vv S_t = \vv M_t$ for momentum and $\vv S_t = \{\vv M_t,\vv V_t\}$ for Adam.
 It is important to note that both \(\vv{M}_t\) and \(\vv{V}_t\) are the same size as the model weights \(\vv{W}_t\), resulting in high memory consumption for large models. This issue is particularly pronounced with Adam, which typically yields the best performance for large language models (LLMs) but incurs the highest memory cost due to the need to maintain both \(\vv{M}_t\) and \(\vv{V}_t\). One key challenge is to retain the high performance of Adam while enhancing its memory efficiency.

%It is an important 
%It has been widely observed that Adam is typically preferred for large language models, while momentum is typically preferred over gradient descent. However, Adam has two copy of momentum states. %Compared with gradient descent and momentum, %Adam %For LLM training in particular, Adam has been widely used, and %For example, %The problem is that the optimizer state $S_t$ could be memory costly. 

\subsection{Static Projected Descent} 
One popular approach to improving memory efficiency is to confine the optimization to a low-dimensional space. To do this, we impose a low rank structure of \(\vv{W} = \vv{\U} \vv{\hat{W}}\), where \(\vv{\U} \in \mathbb{R}^{n \times k}\) is a projection matrix to be determined later and \(\vv{\hat{W}} \in \mathbb{R}^{k \times m}\) is a dimension reduced parameter. When \(k \ll n\), \(\vv{\U}\) and \(\vv{\hat{W}}\) are much smaller in size compared to \(\vv{W}\). Now consider
%
$$
\min_{\vv{\hat{W}}} L(\vv{\U} \vv{\hat{W}}).
$$
%
Applying the optimizer from \eqref{equ:opt} to update \(\vv{\hat{W}}\) along with an optimizer state \(\vv{\hat{S}}\), and mapping the update of \(\vv{\hat{W}}\) back to \(\vv{W}\), we get
%
\bbb  
\vv w_{t+1} = \vv W_t +  \vv \U \phi_t(\vv \hatS_t), 
&& 
 \vv{\hat S}_{t} =  
 \psi_t(\vv {\hat S}_{t-1}, \vv \U \tt \dd L(\vv W_t)),
 \label{equ:static}
\eee  
where we used the fact that 
$\dd_{\vv \hatW} L(\vv \U \vv\hatW) =\vv \U \tt \dd_{\vv W} L(\vv W)$.
This produces a more memory-efficient optimizer, 
as $\vv \hatS_t$ is much smaller than $\vv S_t$ in \eqref{equ:opt} when $k \ll n$.

\subsection{Dynamic Projected Descent} 
With a static $\vv P$, regardless of its values, 
the parameter $\vv W$ is restricted to have a low rank structure. Although the low-rank assumption has been shown to be useful for fine-tuning with LORA-like methods \red{[cite]},  
it is often too limited for pre-training or when the desirable model weights are not inherently low rank. 
 %\eqref{equ:static} obviously fails to solve the original optimization problem in general because $\vv W$ is confined in a fixed lower dimensional space. 

To address this problem, \red{[cite]} 
suggested to keep the projected updated in \eqref{equ:static}, but use different $\vv P$ across the iterations: 
%periodically changes $\vv P_t$ 
%proposed to solve this difficult 
 %One approach to solve this problem is to make the projection matrix  $\vv \U $ 
%change dynamically with $\vv W_t$ and $\vv \hatS_t$, yielding 
\bb
\vv w_{t+1} = \vv W_t +  \vv \U _t \phi_t(\vv \hatS_t), 
&& 
 \vv{\hat S}_{t} =  
 \psi_t(\vv {\hat S}_{t-1}, \vv \U _t \tt \dd L(\vv W_{t})),
 && 
 \vv \U _{t} = \chi_t(\vv \U _{t-1}, \vv W_{t-1}, \vv \hatS_{t-1}), 
 %\label{equ:static}
\ee
where $\chi_t$ is a update rule of $\vv \U _t$ that will be determined in the sequel. 
The intuition is to open up different projection directions at different iterations, so that optimization can be conducted in different subspaces across different iterations. 
This is similar to the update of coordinate descent, except in a continuous fashion.


%all update directions are incorporated in the end when the algorithm is run sufficiently long. 
%every direction is made possible 
%is that we now exhibit different 
%Applying the same optimizer on $\hat W$ %yields 
%consisting of iterative update of form 

%\bb 
% W_{t+1} = W_t + \epsilon  U \phi(S_t, U^+ W_t), 
%&& 
% S_{t+1} =  S_{t} + \epsilon \psi(S_t, U \tt G_t). 
%\ee where $U^+$ is the pseudo inverse of $U$ with $U^+ U = I$, such that $\hat W = U^+ W$.

\begin{exa}
%Dynamic projected descent equipped with 
Gradient descent, momentum and Adam 
with dynamic projection: 
\begin{flalign*}
\text{Gradient Descent}:&~~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t \vv \U _t \vv \U _t\tt \vv G_t,&&
\vv G_t  = \dd L(\vv W_t),  
&&&&&  \\ 
\text{Momentum}: & ~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t  \vv \U _t \vv M_t, &&
\vv M_t = (1-\beta) \vv \U _t\tt \vv G_t + \beta \vv M_{t-1}, &&&&&  \\
\text{Adam}:&~~~~~
\vv W_{t+1} = \vv W_t - \epsilon_t 
\frac{\vv M_t}{\sqrt{\vv V_t} + e}, &&
\vv {\hat G}_t =\vv \U _t \tt  \vv G_t, %\dd L(\vv W_t), 
 &&&&&  \\
&~~~~~
\vv M_t = (1-\beta_{1t})\vv {\hat G}_t + \beta_{1t} \vv M_{t-1},
&& 
\vv V_t = (1-\beta_{2t}) \vv{\hat G}_t^2 + \beta_{2t}\vv V_{t-1}.  &&&&& 
\end{flalign*}
%\red{fix the $t$vs. $t-1$ and $\eta_{2,t}$.}
%The gradient descent, 
\end{exa}


%However, with a static $U$, the optimization is %restricted to a lower dimensional space and hence does not solve the original optimization. 

%It is hence desirable to vary $U$ across iterations, such that optimization can be conducted in different subspaces across different iterations. Let $U_t$ be the projection matrix at iteration $t$,  





%\subsection{Update Rule of $\vv \U _t$}
\paragraph{How should $\vv \U _t$ be updated?}
It is useful to draw intuition from the projected gradient descent rule 
\bbb \vv W_{t+1} = \vv W_t -\epsilon_t \vv \U _t \vv \U _t \tt \vv G_t, ~~~~~~~ \vv G_t = \dd L(\vv W_t), 
\label{equ:gd}
\eee  
in which $\vv \U _t \vv \U _t\tt$ can be viewed as a low rank preconditioning matrix of $\vv G_t$. 
To make it follow the exact gradient descent, we hope to make $\vv \U _t \vv \U _t\tt \vv G_t$ approximate $\vv G_t$ as much as possible. 
In Galore, this is achieved performing 
singular value decomposition (SVD) 
on $\vv G_t$ periodically %via as the left singular vector on $G_t$ in
every $T$ %(say $T=200$) 
iterations: %, e.g., % that is, 
$$
\vv \U_t,~\_, ~\_ = %\mathtt{LeftSingularVector}
\texttt{torch.linalg.svd}
(\vv G_{T\lfloor t/T\rfloor}),
$$
where $T\lfloor t/T\rfloor$ is  the largest multiple of $T$ less than or equal to $t$. 
%
%
However, numerical SVD may incur large computational cost for very large models. Also, since $\vv \U_t$ is fully determined by $\vv G_{T\lfloor t/T\rfloor}$ calculated from a single mini-batch in the last periodic point, it does not incorporate  the gradient information from all data in a timely fashion. 

In this work, we propose to update $\vv P_t$ in a continuous online fashion that incorporates 
the most recent gradient information in a timely fashion, without calling linear algebra routines. 
We view the update of $\vv P_t$ 
as conducting an online principle component analysis (PCA) based on the streaming data of $\{\vv G_t\}$. 

In particular, 
we propose to update $\vv P_t$  at time $t$ by minimizing the following PCA objective:  
\bbb \label{equ:lu} 
L_{\vv G_t}(\vv \U ) = \norm{\vv \U \vv \U \tt \vv{\tilde g}_t - \vv {\tilde g}_t}^2 + \gamma \norm{\vv \U \tt\vv \U  - \vv I_{k\times k}}^2, ~~~~~
\vv{\tilde G}_t = \frac{\vv G_t}{\norm{\vv G_t}}, 
\eee  
where $\norm{\vv A} =\trace(\vv A\tt \vv A)^{1/2}$ is the Frobenius norm and $\vv I_{k\times k}$ is the $k\times k$ identity matrix; we introduced an auxiliary loss to encourage the columns of $\vv \U $ to be orthonormal 
and normalizes $\vv G_t$ to increase stability. 

Note that all stable local minimum of $L_{\vv G_t}(\vv \U )$ is a global minimum,
and $\vv \U $ is a global minimum iff $\vv \U \vv \U \tt \vv {\tilde G}_t$ forms the optimal rank-$k$ approximation of $\vv {\tilde G}_t$ \citep[e.g.,][]{baldi1989neural}, 
and $\vv \U \tt \vv \U = I_{k\times k}$ at optimum when $\eta >0$. 

Instead of minimizing $L_{\vv G_t}(\vv P)$ exactly,
to retain computational efficiency, 
we propose to update $\vv P_t$ by only performing one step of optimization on $L_{\vv G_t} (\vv P)$: 
%one step of optimization on
 %This motivates us to minimize $L_{G_t}\(\vv \U )$ in an online fashion, yielding update rules of form 
$$
\vv \U _{t+1} =\texttt{OptimizerP.step}(\vv P_t, ~~~ \dd L_{\vv G_t}(\vv \U _t)), 
$$
where $\texttt{OptimizerP.step}$ can be a favorite optimizer, such as gradient descent or Adam. 
Note that when using Adam, 
we introduce a copy of optimizer state $\vv S_t^P$ for $\vv \U _t$. 
See Algorithm~\ref{alg:main}. 

%\begin{remark} It is equivalent to replace $\norm{\vv \U \tt \vv \U - \vv I_{k\times k}}^2$ with $\norm{\vv \U \tt\vv \U  - I_{n\times n}}^2$, as they are equivalent upto a constant. \qq{remove}
%\end{remark}


% \subsection{Comparison with Galore \qq{remove}} 
% The recent Galore algorithm \red{cite} and our method share the same essential idea of imposing adaptive projection during optimization 
% to avoid the high memory cost. 
% The key difference is that Galore 
% calculates 
% %Galore is similar to our method, except that 
% $\vv \U_t$ periodically with singular value decomposition (SVD) on $G_t$ in every $T$ (say $T=100$) iterations, that is, 
% $$
% \vv \U_t = \mathtt{SVD}(\vv G_{T\lfloor t/T\rfloor})
% $$
% where $T\lfloor t/T\rfloor$ is  the largest multiple of $T$ less than or equal to $t$. In practice, this is done with \texttt{torch.linalg.svd}.
% Compared with our proposing of having continous updates of $\vv \U_t$, this update is fundamentally discrete. 

% \paragraph{Performance}
% Because $\vv \U_t$ is fully depend on $\vv G_{T\lfloor t/T\rfloor}$ and is freeze for $T$ steps, the information of the more recent $\vv G_t$ is not timely incorporated into $\vv \U_t$. Moreoverall, because $\vv G_t$ is evaluated on a single mini-batch data, it is problematic to have the next $T$ iterations all depend on $\vv \U_t$, which itself depends on a fixed mini-batch data that is rather random. Overall, the step-wise SVD can be viewed as a rather efficient approach to online SVD. 
% %the value of $\vv U_t$, which is used 

% \paragraph{Computational Cost}
% In our case, the update of $\{\vv S_t, \vv \U_t\}$ can be done in parallel, and may not incur slow down at all since each upate of $\vv \U_t$ is cheap. 

% However, the SVD computation of form a bottleneck every $T$ iterations. 
% In addition, the SVD may not scale well when the matrix size is very large. 

% The idea is that we distribute the computation evenly across the iteraitions, and hence can leverage the information more effectively, 
% and is more ammenable for parallelization. 
% %is updated as %$\vv $

% \paragraph{Memory Cost}
% If we update $\vv P_t$ with Adam for the online minimization of $L_{\vv G_t} (\vv P)$, then we incur additional memory cost. ....

% \paragraph{Motivation}
% Galore is motivated by the observation that the gradient in deep learning tends to have a low rank structure. 
% However, as shown in our analysis below, 
% the dynamic projected descent stands as a valid optimization procedure even if the exact gradient exhibit no low rank structure. 

% One key question is the choice of the update rule $\chi_t$ of $\vv \U _t$, 
% and its theoretical implications. 
% In the sequel, we first propose a heusitic rule of updating $\vv \U _t$ as an online PCA problem, 
% then As one of the key theoretical insights, we show that the choice of update rule is surprinsginly flexible and the only essential requirement is that the algorithm should not terminant prematurally when $\dd L(\vv W_t)\neq 0$. 
% \qq{making the point that simply making $\vv P_t$ it is not obvious that we will get "valid" optimizers which would converge to local optima of $L(\vv W)$ at least in the limit of infinitesimal step size. This issue was not addressed in Galore (it only provide analysis of Gradient Descent + Galore with static projection.)}
% %any updates that does not 

\subsection{Hamiltonian Subspace Descent: A Lyapunov Analysis}

\paragraph{Main Difficulty in Theoretical Understanding}
The idea above of projecting an arbitrary optimizer with a dynamically changing $\vv{P}_t$ is heuristic and lacks immediate rigorous theoretical justification. The main challenge lies in the complex interaction between the update of $\vv{U}_t$ and the optimization state $\vv{S}_t$, which could potentially degrade the convergence and other theoretical properties of the original optimizer. A key question is whether we can develop a theoretical framework to understand how $\vv{P}_t$ impacts the optimizer's convergence behavior and provide guidance for the design of the update rules of $\vv{P}_t$.

To gain a grasp of the problem, 
it is useful to  first exam the simple case of projected gradient descent in \eqref{equ:gd} 
which does not have an optimizer state ($\vv S_t = \emptyset$). 
In this case, since $\vv P_t \vv P_t\tt$ is positive semi-finite, 
the update $\vv P_t \vv P_t\tt \vv G_t$ is always non-increasing direction of $L(\vv W)$ for any $\vv P_t$. 
The algorithm is essentially 
a variant of coordinate or subspace descent, 
where $\vv P_t$ defines the subspace on which 
one step of gradient descent is conduced at iteration $t$. 
%
To ensure that \eqref{equ:gd} would find local optima of $L(\vv w)$, 
we mainly need to 
ensure that $\vv P_t \vv G_t = 0$ 
only if $\vv G_t = 0$ to 
prevent the optimizer from stopping  prematurely, 
a mild condition that is satisified e.g., when $\vv P_t$ is updated via (online) PCA on $\vv G_t$. 

This coordinate-descent-like interpretation, however, does not apply to more advanced optimizers that track a momentum state $\vv S_t$. This is because the momentum $\vv S_t$ accumulates the information from the projected gradient $\vv P_{\tau} \vv G_{\tau}$ at all earlier iterations $\tau \leq t$. As $\vv P_t$ changes across time, it is unclear whether the gradient projected to different subspaces would be coherent with each other, and useful for future updates that are conducted in different subspaces. 
%Because
Due to the inertia effect of $\vv S_t$ that 
entangles the information from different subspace together, 
the dynamic behavior here is fundamentally more complicate than naive coordinate descent in which the descent in different subspaces are uncoupled. 


Surprisingly, we show in Section~\ref{sec:layp} 
that the entanglement between $\vv S_t$ and $\vv P_t$ 
\emph{does not} deteriorate the convergence as we worried for a large family optimizers including momentum, Adam and Lion. 
%
%In this section, we present  a continous-time Lyapunov analysis that shows that the update of $\vv \U _t$ can be essentially for a large family optimizzers that yields a Hamlitonian descent structure (cite hamilotonain descent  and Lion paper) \red{todo}. 


We choose to study the dynamic properties of optimizers in the continuous time limit with infinitesimal step size. 
This allows us to abstract away the step size choices and focus on the asymptotic convergence of the algorithm. 
The logic is that 
\emph{
a ``sound" optimizer should be guaranteed to converge to local optima of the loss $L(\vv W)$, 
at least when using sufficiently small step sizes. 
}


As shown in~\citep{chen2023lion, maddison2018hamiltonian}\qq{Lion paper + hamiltonian descent paper}, 
the continuous-time form of many common optimizers 
yields a 
\emph{Hamiltian+Descent} structure,  %in which 
\bbb  \label{equ:hd}
\begin{split}
\ddt \vv W_t =    \partial_{\vv S} H(\vv w_t, \vv S_t) - \Phi(\partial_{\vv W} H(\vv w_t, \vv m_t)) \\ 
\ddt \vv  S_t = -   \partial_{\vv W} H(\vv w_t, \vv S_t) - \Psi(\partial_{\vv S} H(\vv w_t, \vv S_t)),
\end{split} 
\eee  
where $H(\vv W, \vv S)$ is a Hamiltonian (or Lyapunov) function 
that satisfies 
$$
\min_{\vv S} H(\vv W, \vv S) = L(\vv W), ~~~~\forall \vv W, 
$$
so that minimizing $L(\vv W)$ reduces to $H(\vv W, \vv S)$;
and $\Phi(\cdot), \Psi(\cdot)$ are two monotonic mappings satisfying 
\bb 
\norm{\vv X}_{\Phi}^2 \defeq \langle\vv X,  \Phi(\vv X)\rangle\geq0, && 
\norm{\vv X}_{\Psi}^2 \defeq \langle\vv X,  \Psi(\vv X)\rangle\geq0, &&
\forall \vv X.
\ee 
It is easy to see that the system in \eqref{equ:hd} decreases $H(\vv W, \vv S)$ monotonically: 
%because 
\bbb  \label{equ:dh}
\begin{split}
\ddt H(\vv W_t, \vv S_t)
& = \llangle \partial_{\vv W} H_t, \ddt \vv W_t\rrangle + \llangle \partial_{\vv S} H_t, \ddt \vv S_t\rrangle  \\ 
& =\llangle \partial_{\vv W} H_t,  
  \partial_{\vv S} H_t - 
 \Phi(\partial_{\vv W} H_t ) 
 \rrangle + \llangle \partial_{\vv S} H_t, -  \partial_{\vv W} H_t - 
 \Psi(\partial_{\vv S} H_t )  \rrangle  \\  
& = - \norm{\partial_{\vv W} H_t}_{\Phi}^2- \norm{\partial_{\vv S} H_t}_{\Psi}^2 \leq 0, 
%- \llangle \partial_{\vv W} H_t,     \Phi_t(\partial_{\vv W} H_t ) 
 %\rrangle - \llangle \partial_{\vv S} H_t,   \Psi_t(\partial_{\vv S} H_t )  \rrangle 
 %\leq 0, 
 \end{split}
 \eee  
 where we write 
 $\partial_{\vv W} H_t = \partial_{\vv W}H(\vv W_t, \vv S_t) $ and similarly for $\partial_{\vv S} H_t$. The main idea is that the cross terms are canceled, leaving on the negative terms. 
 %= \partial_{\vv W}H(\vv W_t, \vv S_t) $.%
 

\begin{exa}
The momentum method yields 
following continuous-time form and  Hamiltonian: 
\bb 
\ddt  \vv w_t = - \vv m_t, 
&&&&& 
\ddt  \vv m_t =a (\dd L(\vv w_t) - \vv m_t), 
&&&&&&
\text{with}~~~~~~
H(\vv W, \vv  M) = 
 L(\vv W) + \frac{\norm{\vv M}^2}{2a},
\ee
%The continuous-time Adam and its Ham
Adam yields the following continuous-time form and Hamiltonian, 
\bb 
\ddt {\vv W_t} = \frac{\vv m_t}{\sqrt{\vv v_t}+e},   && 
\ddt{\vv m}_t = a(\dd L(\vv w_t) - \vv m_t), && \ddt \vv v_t = b(\dd L(\vv w_t)^2 - \vv v_t), 
\ee
\bb 
\text{with}~~~~~~
H(\vv W, \vv m, \vv v) 
= L(\vv w) + \frac{1}{2a}
\llangle \frac{\vv M}{\sqrt{\vv V} +e}, ~ \vv M\rrangle. 
 \ee 
We have $\ddt H(\vv W_t, \vv m_t, \vv v_t)  \leq 0$
 when $a \geq  b/4$. 
%The projected version
\end{exa}

\begin{exa}
The Lion-$\mathcal K$ optimizer of \red{cite} (without weight decay) is 
%yields 
\bb 
\ddt \vv W_t = \dd \mathcal K (b\vv M_t -  (1-b)(\dd L(\vv W_t)+\vv M_t)),&& 
\ddt \vv M_t = -a ( \dd L(\vv W_t) + \vv M_t), 
\ee 
One of its Hamiltonian (Eq~(13) in \red{lion K paper}) is 
$$
H(\vv W, \vv M) = a L(\vv W) +  \frac{1}{b} \mathcal K(b  \vv M). 
$$
\bb 
\ddt H(\vv W_t, \vv M_t)
& =  a
\langle  \vv G_t, \dd \mathcal K (b \vv{M}_t - (1-b) \vv \Delta_t) 
\rangle  
- a \langle \dd \mathcal K(b \vv M_t), \vv G_t + \vv M_t  \rangle 
\ee 
\end{exa}

\subsection{Hamiltonian Subspace Descent}  
Applying dynamic projection to Hamiltonian descent in \eqref{equ:hd}, 
we obtain the following family of 
%For optimizers
\bbb \label{equ:hadyp}
\begin{split}
& \ddt \vv W_t =    \vv \U_t \partial_{\vv \hatS} H(\vv w_t, \vv \hatS_t) - \Phi(\partial_{\vv W} H(\vv w_t, \vv m_t))  \\
&\ddt \vv  \hatS_t = -     \vv \U_t\tt \partial_{\vv W} H(\vv w_t, \vv \hatS_t) - \Psi(\partial_{\vv \hatS} H(\vv w_t, \vv \hatS_t)) \\
&\ddt \vv \U_t = \Gamma(\vv \U_t, 
 \dd L(\vv W_t), \vv W_t, \hatvv S_t), 
 \end{split}
\eee  
where $\Gamma $ is an update rule of $\vv P_$. 
Following essentially the same derivation as \eqref{equ:dh}, 
one can show that $H(\vv W, \vv S)$ remains an Lyapunov function of \eqref{equ:hadyp}, regardless of the choice of $\Gamma$: 
%It yields the same Lyapunov function, 
\bb
\ddt H(\vv W_t, \hatvv S_t)
& = - \norm{\partial_{\vv W} H_t}_{\Phi}^2- \norm{\partial_{\vv S} H_t}_{\Psi}^2 + 
\langle \partial_{\vv W} H_t, \vv P_t \partial_{\hatvv S } H_t \rangle 
- \langle \partial_{\hatvv S} H_t, \vv P_t\tt  \partial_{\vv W} H_t \rangle \\ 
& = - \norm{\partial_{\vv W} H_t}_{\Phi}^2- \norm{\partial_{\vv S} H_t}_{\Psi}^2 \leq 0, 
%= - \llangle \partial_{\vv W} H_t,    \Phi(\partial_{\vv W} H_t ) \rrangle - \llangle \partial_{\vv S} H_t,  \Psi(\partial_{\hatvv S} H_t ) \rrangle  \leq 0. 
\ee
where we use the  key adjoint property of $\vv P$ and $\vv P\tt $ that  $\langle \vv P_t \vv X, \vv Y\rangle = 
\langle \vv X, \vv P_t\tt \vv Y\rangle$, which allows us to cancel the crossing terms. 
%This is because the $\vv P_t$ only impacts the crossing term, which is canceled away when calculating $\ddt H(\vv W_t, \hatvv S_t)$. 
%See Appendix \red{ddd} for detailed derivation, where we show that the key is the adjoint property of $\vv P$ and $\vv P\tt $ that  $\langle \vv P_t \vv X, \vv Y\rangle = \langle \vv X, \vv P_t\tt \vv Y\rangle$. 
\begin{exa}
Momentum + {dynamic subspace descent} is 
%The momentum+{\name} method is %ynamic projection is 
\bb
\ddt \vv w_t = -\vv \U_t \vv m_t , && \vv{\hat g}_t = \vv \U_t\tt  \dd L(\vv w_t), && \ddt \vv {\hat m}_t = a (\vv{\hat g}_t - \hatvv m_t). 
\ee 
It yields a Lyapunov function of form
$$
H(\vv w, \vv m) = L(\vv w) + \frac{\lVert {\vv{\hat M}\rVert}^2}{2a}. 
$$
for which we have 
\bb 
\ddt H(\vv w_t,\vv {\hat m}_t) 
& = - a \dd L(\vv w_t) \tt \vv \U_t \hatvv m_t + a \hatvv m_t\tt (\vv \U_t\tt \dd L(\vv w_t) -\hatvv  m_t) 
 = - a \norm{\vv m_t}_2^2\leq0.
\ee 
\end{exa}

\begin{exa}
Adam + {dynamic subspace descent} is 
\bb 
\ddt \vv w_t =  \vv \U_t \frac{\hatvv m_t}{\sqrt{\hatvv v_t}+e},   &&  \vv{\hat G}_t =  \vv \U_t \tt \dd L(\vv w_t), && 
\ddt \hatvv m_t = a(\vv{\hat g}_t - \hatvv m_t), && \ddt \hatvv v_t = b(\vv {\hat g}_t^2 -\hatvv  v_t). 
\ee 
It yields a Lyapunov function when $a > b/4$, 
\bb 
H(\vv W, \vv m, \vv v) 
= L(\vv w) + \frac{1}{2a}
\left \llangle \frac{\hatvv M}{\sqrt{\hatvv V} +e}, ~ \hatvv M \right \rrangle. 
\ee 
%H(x, m, v) = a f(x) + \frac{1}{2}  \left(\frac{1}{\sqrt{v} +e}\right)\tt m^2. 
%for which $\ddt H(x_t, m_t, v_t) \leq 0$ when $a \geq \frac{b}{4}$: 
\bb 
& \ddt H(\vv w_t, \hatvv m_t, \hatvv v_t)  \\ 
& = -\llangle \vv g_t, \vv \U_t \frac{\hatvv m_t}{\sqrt{\hatvv v_t}+e} \rrangle 
+ \frac{1}{a}\llangle 
\frac{\hatvv m_t}{\sqrt{\hatvv v_t} + e},~~ a (\vv \U_t\tt  \vv g_t -\vv m_t) \rrangle 
-  \frac{b}{4a } \llangle\frac{\vv m_t^{\odot 2}}{ \sqrt{\hatvv v_t}\odot (\sqrt{\hatvv v_t} + e)^{\odot 2}},~~ (\vv{\hat g}_t^{\odot 2} - \hatvv v_t) \rrangle \\ 
& = 
- \llangle  1 - \frac{b}{4a}\frac{\sqrt{\hatvv v_t}}{\sqrt{\hatvv v_t} + e},~ \frac{
\hatvv m_t^{\odot 2}}{\sqrt{\hatvv v_t }+ e} \rrangle 
-  \frac{b}{4a} \llangle \frac{\hatvv m_t^{\odot 2} }{ \sqrt{\hatvv v_t}\odot (\sqrt{\hatvv v_t} + e)^{\odot 2}} , ~ \hatvv G_t^{\odot 2} \rrangle   \\ 
& \leq 
- \left(1 - \frac{b}{4a}\right) 
 \norm{\frac{\hatvv m_t}{\sqrt{\sqrt{\hatvv v_t }+ e}}}^2 - \frac{b}{4a} \norm{ \frac{\hatvv m_t \hatvv g_t}{ \sqrt[4]{\hatvv v_t}{(\sqrt{\hatvv v_t} + e})} }^2  \leq 0, 
%&  = (a-\frac{b}{4})
\ee 
where we assume $a \geq b/4$. 
\end{exa}

\begin{exa}
\red{Lion}

\end{exa}

\subsection{Convergence to Local Optima}
In addition to the Lyapunov structure, 
to make system \eqref{equ:hadyp} a sound optimizer 
we need to impose additional conditions to ensure that it has the right set of invariant set, so that it gurantes the local optima of Lyapunov function. 
%Having a Laypunov function 

Assume $H(\vv W, \hatvv  S)$ is a smooth Lyapunov function with $\ddt H(\vv W_t,\hatvv S _t)\leq 0$, we have by LaSalle's invariance principle that the set of accumulation points of any trajectory is contained in ${\mathcal I}$ where ${\mathcal I}$ is the union of complete trajectories contained entirely in the set $ \{\vv W_t, : \ddt {H}( \vv W_t,\hatvv S _t) = 0 \}$.  


\begin{ass}\label{def:ad}
%Consider 
%Assume 
%We call that
Assume the functions in 
system \eqref{equ:hadyp} are continously differentiable and 
%is  if %satisfies the following assumption: 

i) $\ddt H(\vv W_t, \hatvv S_t) =0$ implies $\hatvv  G_t =  \vv P_t\tt \dd L(\vv W_t) =0$ and $\ddt W_t = 0$. 

ii) 
When  $\vv G_t \equiv \vv G\neq 0$,
%the null set 
the set 
$\{\vv P \colon \vv P\tt \vv G  = 0\}$ is not a positive invariant set of $\ddt \vv \U_t = \Gamma(\vv \U_t, \vv G_t)$. 
\end{ass}

This is a mild condition. 
Assumption i) holds 
for the typical optimizers converges to the local optima of $L(\vv W)$,
and Assumption ii) ensures that it is impossible to have $\P_t \tt \vv G = 0$ 
%ensures that 
%is obviously satisfied for 
%It is satisfied, for example, 
%whenever ...
%The analy

\begin{thm}
Assume Assumptition~\ref{def:ad} holds. 
%Assume \eqref{hadyp} is admissible,
%and all functions involved in \eqref{hadyp} are continuously differentiable, an
Let 
$(\vv W_t, \vv S_t, \vv P_t)_{t}$ 
be a bounded solution of \eqref{equ:hadyp}, % that is confined in a bounded set,  
%and the update rule of $\vv P_t$ is admissible. 
then all the accumulation points $\{\vv W_t \}$ as $t\to +\infty$ 
are stationary points of $L(\vv W)$. 
%positive limit set of the $W_t$
%Let $\mathcal L$ be the set of local optima of $L(\vv W),$ then $\vv W_t\to \mathcal L$ as $t\to +\infty$.  
\end{thm}
\begin{proof}
%Let $\{(W, )\}$
By LaSalle's invariance principle,
the positive limit set of $(\vv W_t, \vv S_t, \vv P_t)_{t}$ must be contained in $\mathcal I,$ where 
%the bounded trajectories of the 
%the system must converges to the maximum invariant set of 
$$\mathcal{I} = 
\{\text{the union of complete trajectories 
satisfying $ \ddt H(\vv W_t, \hatvv S_t) =0$, $\forall t$ 
}\}.
$$
%the maximum invariant set inside $\mathcal X = \{(\vv W, \hatvv S, \vv P) \colon \ddt H(\vv W_t, \hatvv S_t, \vv P_t) =0 \}$.   $$

From the Assumption i),
the trajectories contained in 
 $\mathcal I$ must satisfy 
 $\ddt W_t = 0$, which implies 
 $\ddt \vv G_t = \ddt \dd L(\vv W_t) = 0$ and $\hat G_t = 0$ and hence 
 %$\hatvv  G_t =  \vv P_t\tt \dd L(\vv W_t) = 0$, and $\ddt \vv W_t = \ddt \vv G_t = 0$, which means that  
 $\vv G_t \equiv \vv G$ is a constant with $\P_t\tt \vv G =0$. 
 Moreover, from Assumption ii), 
 we must have $\dd L(\vv W_t) = \vv G_t\equiv 0$, since otherwise the trajectory is not invariant. As a result,
 all trajectories in limit set $\mathcal I$ must have $\dd L(\vv W_t) = 0$. Because $\dd W_t=0$, 
 these trajectories are points for static points for  $\vv W_t$. 
 %inside the limit set. 
\end{proof} 



 

==> tex/notes.tex <==

\section{More Lyapunov Analysis}

\paragraph{Gradient Descent + Moving Subspaces} 
For simplicity, 
Assume the gradient matrix $G_t$ is of size  $G_t \in \RR^{d_1 \times d_2}$. 
Let us consider 
\bb 
\ddt  \vv W_t =  -\vv  \U_t \vv \U_t\tt \vv G_t, 
~~~~~ \vv G_t = \dd L(\vv W_t), 
\ee 
where $\vv P_t$ is updated in any fashion that the renders the ODE to have well defined solutions. 
%where $U_t \in \RR^{d_1 \times k}$ is any matrix, updated in any fashion. 
%This forms a rank-$k$ approximation of the exact gradient $G_t$.%There is no practical reason to do this since there is no gradient to save. But let us start with it for motivation.  
Because $\vv \U_t \vv \U_t\tt$ is positive semi-definite, the objective is always non-increasing: 
%We have:  
\bb 
\ddt L(\vv W_t) =  -\trace( \vv \U_t \vv \U_t\tt \vv G_t \vv G_t\tt) = -\norm{\vv \U_t\tt \vv G_t}^2 \leq 0.
\ee 
However, the algorithm may determinant 
if $\vv \U_t \vv G_t = 0$, even if $\vv G_t \neq 0$. 
To avoid this, we should update $\vv P_t$  in a way that ensures that 
%This shows that any choice of $U_t$ would yield descent. 
%However, this is not sufficient to ensure that the %algorithm will converge to a local optima of $f$. 
%This is because we would need to ensure that 
\bbb \label{equ:dd}
\vv \U_t\tt\vv G_t= 0 
&& \implies 
&&\vv G_t = 0 
\eee 
One way to ensure this is to set $\vv \U_t $ to the top left singular vector of $\vv G_t$, or equivalently top eigenvectors of $\vv G_t\vv G_t\tt$. 
However, since the requirement in \eqref{equ:dd} is very mild, one can update $\vv P_t$ with a fast and rough approximation of PCA or SVD, rather than the expensive exact version. 


One way to formulate this is that 
$$
U_t = \argmin_{U} \norm{U U \tt G _t - G_t}^2_F, 
$$
which minimizes the difference between the low rank projected gradient $U U \tt G$ with the exact gradient $G$. 

Theoretically, such the optimal $U_t U\tt $ forms the optimal rank-$k$ approximation of $G_t$, and $U_t$ spans the subspace of the top eigenvectors of $G_t G_t\tt$. 

To save computation, we use the amortized update: 
$$
\dot U_t = - \dd {\norm{U U \tt G _t - G_t}^2_F} 
$$


A different way. Note that 
\bb
\ddt \norm{U_t}_F^2/2 &  =   - \trace( (U_tU_t\tt-I)G_tG_t\tt U_t U_t\tt )  \\
& = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) + \trace(G_t G_t\tt U_t U_t\tt). 
\ee
Hence, define a Lyapunov function $H(X_t, U_t) = f(X_t) + \norm{U_t}_F^2$. We have 
\bb
\ddt (f(X_t) + \norm{U_t}_F^2) = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) \leq 0. 
\ee

\paragraph{+ Momentum }

Let us consider 
\bb 
& \dot U_t = - (U_tU_t\tt-I)G_tG_t\tt U_t \\ 
& \dot X_t = - U_t M_t \\ 
& \dot M_t =  U_t\tt G_t - \beta  M_t
\ee 

\bb 
\ddt f(X_t) =  -\trace( U_t M_t G_t\tt) \leq 0.
\ee 


\bb 
\ddt \norm{M_t}_F^2 /2 & = \trace (U_t\tt  G_t M_t\tt ) - \beta \norm{M_t}_F^2 \\
& = \trace(M_t G_t\tt U_t) - \beta \norm{M_t}_F^2 \\
& = \trace(U_t M_t G_t\tt ) - \beta \norm{M_t}_F^2
\ee 

Hence, 
\bb 
\ddt (f(X_t) +  \norm{M_t}^2_F/2) = - \beta \norm{M_t}^2_F. 
\ee 

However, the minimum may not strictly optimize $f$. 

At the fixed point, we have 
\bb 
U_t M_t = 0, ~~~~~~ U_t\tt  G_t - \beta M_t = 0.
\ee  
This gives $U_t U_t \tt G_t = 0$.
In this case, the fixed point condition on $U_t$ is 
$$
\dot U_t  =  G_t G_t\tt U_t = 0.
$$


\bb
\ddt \norm{U_t}_F^2 /2&  =   - \trace( (U_tU_t\tt-I)G_tG_t\tt U_t U_t\tt )  \\
& = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) + \trace(G_t G_t\tt U_t U_t\tt). 
\ee
Hence, 
\bb
\ddt (f(X_t) + \norm{U_t}_F^2) = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) \leq 0. 
\ee

\subsection{Lagrangian}

\paragraph{+ Gradient Descent}

Consider  the eigen problem on $GG\tt$: 
$$
\max_{U} U\tt G G\tt  U ~~~s.t.~~~ \norm{UU\tt-I}^2 = 0.
$$

The Langrangian update is 
\bb 
\dot U_t = G G \tt U - \lambda_t (UU\tt-I) U \\ 
\dot \lambda_t = \norm{UU\tt-I}^2. 
\ee 

Let us consider 
\bb 
\dot U_t = - \dd \phi_t(U_t) \\
\dot \lambda_t = 
\dot X_t =  - U_t  U_t\tt G_t
\ee 

\bb 
\ddt f(X_t) =  -\trace( U_t U_t\tt G_t G_t\tt) \leq 0.
\ee 

This shows that any choice of $U_t$ would yield descent. But it may not result in the local optima of $f$. 

To leverage the update of $U_t$: 

\bb
\ddt \norm{U_t}_F^2/2 &  =   - \trace( (U_tU_t\tt-I)G_tG_t\tt U_t U_t\tt )  \\
& = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) + \trace(G_t G_t\tt U_t U_t\tt). 
\ee
Hence, 
\bb
\ddt (f(X_t) + \norm{U_t}_F^2) = - \trace(U_t U_t\tt G_tG_t\tt U_t U_t\tt ) \leq 0. 
\ee

\subsection{+Adam}
Recall the Lyapunov function of Adam: 
\bb 
& \dot m_t = \dd f - \alpha_1 m_t \\
& \dot v_t = \dd f^2 - \alpha_2 v_t \\
& \dot x_t = - m/\sqrt{v_t}
\ee 
Consider 
$$
H = f(x)  +  \sum \frac{ m_t^2}{2 \sqrt{v_t}} 
$$

\bb 
\ddt H 
& =-  \dd f \tt m /\sqrt{v_t} + (m /\sqrt{v} ) \tt (\dd f - \alpha_1 m_t) + -(\frac{1}{2}(m_t)^2 /(v_t)^{3/2} )\tt  (\dd f^2 - \alpha_2 v_t)  \\
& =- (\alpha_1 - \alpha_2 /2 ) (m /\sqrt{v} ) \tt ( \alpha_1 m_t)  - (\frac{1}{2}(m_t)^2 /(v_t)^{3/2} )\tt  \dd f^2  \leq 0 ~~~~\ant{if $\alpha_1 \geq \alpha_2/2$}
%- \alpha_2 v_t)  
\ee 

Consider the subspace version: 
\bb 
& U_t =\text{ any update} \\ 
& \dot m_t =  (U_t \dd f) - \alpha_1 m_t \\
& \dot v_t =  (U_t\dd f)^2 - \alpha_2 v_t \\
& \dot x_t = - U_t \tt m/\sqrt{v_t}
\ee 
Consider 
$$
H = f(x)  +  \sum \frac{ m_t^2}{2 \sqrt{v_t}} 
$$

\bb 
\ddt H 
& =-  \dd f  \tt U \tt  m /\sqrt{v_t} + (m /\sqrt{v} ) \tt (U \dd f - \alpha_1 m_t) + -(\frac{1}{2}(m_t)^2 /(v_t)^{3/2} )\tt  ((U\dd f)^2 - \alpha_2 v_t)  \\
& =- (\alpha_1 - \alpha_2 /2 ) (m /\sqrt{v} ) \tt ( \alpha_1 m_t)  - (\frac{1}{2}(m_t)^2 /(v_t)^{3/2} )\tt  (U \dd f)^2  \leq 0 ~~~~\ant{if $\alpha_1 \geq \alpha_2/2$}
%- \alpha_2 v_t)  
\ee 


Consider 
$$
\phi(U) = \norm{U U\tt G - G}_F^2  + \gamma \norm{U U \tt - I}^2_F.
$$

\bb 
\dot U_t 
& =  - (UU\tt G - G) G \tt U  - \gamma (U U \tt - I ) U \\ 
& =  -\left( UU\tt G  G\tt U - G G\tt U 
  + \gamma (U U \tt  U - U) \right) \\
  & =  - \left( 
(  UU\tt - I)(G G\tt U + \gamma U)
  \right) \\
  & = - (U U \tt - I)(GG \tt + \gamma I) U.
\ee 

Consider $\gamma = 0$ for now: 
$$
\dot U_t = - (U_tU_t\tt-I)G_tG_t\tt U_t. 
$$



\section{Online PCA}

%be a positive definite matrix. 
The following algorithm learns the subspace of the top $k$ left singular vectors of $\vv G$:  
$$
\min_{\vv \U} L_{\vv G}(\vv \U) =
 \frac{1}{2}\norm{\vv \U \vv \U\tt  \vv G- \vv G}^2.
$$
\begin{lem}
The gradient of $L_{\vv G}$ is 
\bb
\dd L_{\vv G}(\vv \U) & =  (\vv \U \vv \U\tt \vv G - \vv G ) \vv G \tt \vv \U + \vv G (\vv G \tt \vv \U \vv \U\tt - \vv G\tt ) \vv \U \\
%& = \vv \U \vv \U \tt\vv  A \vv \U + \vv A \vv \U \vv \U\tt \vv \U - 2 \vv A \vv \U \\
& = (\vv \U\vv \U\tt - \vv I) \vv A\vv \U + \vv  A\vv \U (\vv \U\tt \vv \U - \vv I)  \ant{$\vv A  = \vv G \vv G\tt$.}
\ee 
\begin{proof} 
Linearization of $L_{\vv G}(\vv \U + \vv \Delta)$ around $\vv \U$ yields 
\bb 
L_{\vv G}(\vv \U + \vv \Delta) - L_{\vv G}(\vv\U)   
& \approx  \trace((\vv \U \vv \U\tt \vv G - \vv G) ( \vv \Delta \vv \U\tt\vv G + \vv \U  \vv \Delta\tt\vv G ) \tt )  \\
& = \trace((\vv \U \vv \U\tt \vv G - \vv G)\vv G\tt \vv \U  \vv \Delta \tt )  + \trace( (\vv \U \vv \U\tt G - \vv G) \vv G\tt  \vv \Delta \vv \U \tt)   \\
& = \trace((\vv \U \vv \U\tt \vv G - \vv G)\vv G\tt \vv \U  \vv \Delta \tt )  + \trace( \vv P\tt (\vv \U \vv \U\tt G - \vv G) \vv G\tt  \vv \Delta \vv )   \\
& = \trace\left ( \left ((\vv \U \vv \U\tt \vv G - \vv G)\vv G\tt \vv \U   + 
\vv G (\vv G \tt \vv \U \vv \U\tt  - \vv G\tt ) \vv P  \right ) \vv \Delta\tt \right ) . 
%& = \trace((\vv \U \vv \U\tt \vv G - \vv G) \vv G\tt \vv \U  \vv \Delta \tt )  + \trace(  \vv \Delta \tt \vv G (\vv G \tt \vv \U \vv \U\tt - \vv G \tt ) \vv \U )  \\
\ee 
Reading out the linear coefficient of $\vv \U$, we have
\bb
\dd L(\vv \U) & =  (\vv \U \vv \U\tt \vv G - \vv G ) \vv G \tt \vv \U + \vv G (\vv G \tt \vv \U \vv \U\tt - \vv G\tt ) \vv \U. 
%& = \vv \U \vv \U \tt\vv  A \vv \U + \vv A \vv \U \vv \U\tt \vv \U - 2 \vv A \vv \U \\
%& = (\vv \U\vv \U\tt - \vv I) \vv A\vv \U + \vv  A\vv \U (\vv \U\tt \vv \U - \vv I) 
\ee 
\end{proof} 


The update is 
$$
U \gets U + \epsilon (2 AU -  AU U\tt U - U U \tt A U)
$$
Or the ODE: 
$$
\dot U_t = 2 A U_t - (A U_tU_t\tt U_t + U_tU_t\tt A U_t)
$$
Plugging $A = GG\tt$, 
$$
\dot U_t = 2  G G\tt  U_t - (GG\tt U_tU_t\tt U_t + U_tU_t\tt GG\tt U_t)
$$
\paragraph{Preserving the orthonormality} 
\begin{thm}
If $U\tt U= I$ at some point, then the dynamics will keep it. 
Moreover, we in fact have 
$$
\ddt (\norm{I - U\tt U}^2_F/2) = - 4 \trace((Q - I) \tt U\tt A U (Q - I)) \leq 0,
$$
where $Q = U\tt U$. 
\end{thm} 
\begin{proof} 
\bb 
\ddt (U\tt U) &  = \dot U \tt U + U \tt \dot U \\
& = (2 A U_t - (A U_tU_t\tt U_t + U_tU_t\tt A U_t)) \tt U_t
+ U_t\tt (2 A U_t - (A U_tU_t\tt U_t + U_tU_t\tt A U_t)) \\
& = 2 U\tt A U - U\tt U U\tt  A\tt U - U\tt A\tt U U\tt U + 2 U \tt A U - U\tt A U U \tt U - U\tt U U\tt A U  \\
& = 4 U\tt A U  - U\tt U  U \tt A\tt U - U\tt A\tt U U\tt U  - U\tt A U U \tt U - U\tt U U\tt A U  \\
\ee 
Since $A = A\tt$, we have 
\bb 
\ddt (U\tt U) 
&  = 4 U\tt A U  -2  U\tt U U \tt A\tt U - 2 U\tt A\tt U U\tt U  \\
&  = 4 U\tt A U  -2  U\tt
 ( U U \tt A   - A U U\tt ) U 
 % - U\tt A U U \tt U - U\tt U U\tt A U  \\
\ee 
Assume we already have $U\tt U = I$, then 
$$
 4 U\tt A U  -2  U\tt
 ( U U \tt A   - A U U\tt ) U 
 =  4 U\tt A U  -2 U\tt A U - 2 U\tt A U = 0.
$$
Therefore, $U\tt U=I$ is a fixed point. 
\end{proof}

Let $Q = U \tt U$, we have
$$
\dot Q = 2(I - Q) U \tt A U   + 2 U\tt  A U (I - Q)
$$
Hence, 
\bb
\ddt( \norm{I - Q}^2/2) &  = \trace(( Q - I) \tt \dot Q) \\
& = - 2\trace((Q-I) \tt (I - Q) U \tt A U)  -  2\trace( (Q - I)\tt  U\tt  A U (I - Q) ) \\
& = - 4 \trace((Q - I) \tt U \tt A U (Q - I)) \leq 0.
\ee


\paragraph{Particle wise update }
Let $U = [u_1, \ldots, u_k]$, then we can write the update into 
$$
\dot u_i = 2 A u_i - \sum_j A u_j u_j\tt u_i - \sum_j u_j u_j \tt A u_i 
$$
Reduced to 
$$
\dot u_i = 2 A u_i - \sum_{j=1}^k  (u_i \tt A  u_j ) u_j -  \sum_j   (u_i\tt  u_j) A u_j 
$$
%The update can be writting into 

